Mechanism of current-assisted Bloch-point wall stabilization for ultra fast dynamics

Two types of domain walls exist in magnetically soft cylindrical nanowires: the transverse-vortex wall (TVW) and the Bloch-point wall (BPW). The latter is expected to prevent the usual Walker breakdown, and thus enable high domain wall speed. We showed recently [M. Sch\"obitz \etal, Phys. Rev. Lett. 123, 217201 (2019)] that the previously overlooked OErsted field associated with an electric current is a key in experiments to stabilize the BPW and reach speed above 600 m/s with spin-transfer. Here, we investigate in detail this situation with micromagnetic simulations and modeling. The switching of the azimuthal circulation of the BPW to match that of the OErsted field occurs above a threshold current scaling with $1/R^3$ ($R$ is the wire radius), through mechanisms that may involve the nucleation and/or annihilation of Bloch points. The domain wall dynamics then remains of a below-Walker type, with speed largely determined by spin-transfer torque alone.

==> commands_equations.tex <==
%My commands for equations
\newcommand{\sscf}[1]{#1(\boldsymbol{r})} %steady scalar field (r)
\newcommand{\scf}[1]{#1(\boldsymbol{r},t)} %scalar field (r,t)
\newcommand{\svf}[1]{\boldsymbol{#1}(\boldsymbol{r})} %steady vector field
\newcommand{\vf}[1]{\boldsymbol{#1}(\boldsymbol{r},t)} %vector field (r,t)
\newcommand{\heff}{\mathbf{H}_{eff}}
\newcommand{\hd}{\boldsymbol{H}_{d}}
\newcommand{\hzee}{\boldsymbol{H}_{zee}}
\newcommand{\ve}[1]{\mathbf{#1}}
\newcommand{\uv}[1]{\hat{\boldsymbol{#1}}}
\newcommand{\pdt}[1]{\frac{\partial #1}{\partial t}}
\newcommand{\fd}[2]{\frac{\delta #1}{\delta #2}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dv}[2]{\frac{d #1}{d #2}}
